Interplay between cortical adhesion and membrane bending regulates microparticle formation

The formation of microparticles requires the bending of the plasma membrane away from the cytosol. The capcity of the cell membrane to form a microparticle, and the rate of membrane deformation, are controlled by multiple factors, including loss of lipid asymmetry (primarily the exposure of phosphatidylserine on the outer leaflet), detachment of the membrane from the cortical cytoskeleton, and bleb expansion due to pressure. In this work, we develop a biophysical model that accounts for the interaction between these different factors. Our findings reveal that the linkage between the membrane and cortex is a key determinant of outward budding. Ultimately, the rates and mechanical parameters regulating cortical linkage interact with the kinetics of phosphatidylserine flipping, laying out a mechanical phase space for regulating the outward budding of the plasma membrane.

==> Notes.tex <==
Literature review in a month or two on microvesicle importance 

\subsection*{Size}
The size of extracellular vesicles (EVs) can range from 0.03-1 $\mu$m in diameter (In contrast, for instance, human red blood cells are on the scale of 7-10 $\mu$m), and they are released from many cells under normal conditions.
Their further classification as microparticles or exosomes depends on their origin story.
For exosomes, which originate as intracellular vesicles which fuse with the plasma membrane and release their contents into the extracellular space (as in the release of neurotransmitters), exosome size can be correlated to small increases in membrane capacitance as each fusion event results in a step-wise increase in membrane area \cite{almers1990exocytosis}.
Presumably this logic could be inverted -- the loss of membrane associated with the formation of microparticles would result in a step-wise decrease in capacitance. 
Interestingly, the scale and shapes of red blood cells varies and changes over life stages in amphibians, and as elegantly illustrated by Gulliver, there is a great deal of variation in size and morphology across taxa. 

Microparticles can be isolated using a variety of methods, many of which, for instance centrifugation, rely on particle size \cite{kano2019extracellular}.

%\begin{figure}[b!]
%    \centering
%    \includegraphics[width=50mm,scale=0.5]{Figures/Mi%    \caption{Microparticles encompass a broad range of sizes.}
%    \label{fig:MicroparticleSketchl}
%\end{figure}

\subsection*{Speed}
How quickly does the fusion of a vesicle with the plasma membrane occur, and what can we learn about the fusion process from its time constraints?
Almers clearly lays out reasoning in a lovely review on exocytosis \cite{almers1990exocytosis} which is summarized below. 
Neurons are a prime system to consider this question.
Intracellular vesicles containing transmitters are located close to the presynaptic plasma membrane.
When neighboring (~10-20 nm) calcium channels open and the local concentration of calcium increases the fusion of these vesicles with the membrane, their release into the synapse and their interaction with the postsynaptic receptors that trigger the neighboring neuron.
Based on a postsynaptic delay of 0.5 ms in neurons, it can be concluded that the fusion of intracellular vesicles carrying transmitters with the membrane, which is only one component of this process, must occur in less than 0.5 ms. 
How much many steps in a biocehmical cascade could occur in this time frame to elicit vesicle fusion with the membrane? 
The author concludes that in the fast exocytosis occuring in some neurons, there is only time for the conformational change of a single molecule type to facilitate vesicle fusion with the membrane \cite{almers1990exocytosis}. 

\subsection*{Synthesis of lipid bilayers}
Lipids are synthesized within the endoplasmic reticulum (ER) and incorporated into a membrane there. 
Transmembrane proteins are incorporated into the membrane of the ER midway through their synthesis such that their final assembly takes place within the membrane of the ER.

\subsection*{Composition}
The plasma membrane has spatial organization with lateral lipid rafts (10-200 nm patches enriched in sterols and sphingolipids that in total comprise about 30\% of the membrane \cite{pike2009challenge}) and transmembrane components. 
Spatial heterogeneity (\textit{e.g.} lipid rafts, membrane molecules like surface antigen receptors, transmembrane proteins, etc., and positive and negatively charged outer and inner leaflets, respectively) in the membrane allows for the formation of microparticles with different profiles of membrane components, and functional implications \cite{hugel2005membrane}. 
Many microparticles and membrane enveloped viruses depend on lipid rafts and cholesteral, which is increased in the raft, for their formation \cite{del2005tissue}. 
I presume this includes the intracellular/intraparticle composition, in addition to membrane composition. 

The plasma membrane is composed of two layers of phospholipids -- the inner and outer leaflets.
The hydrophilic phosphate side of the lipids interfaces with the the watery interior of the cell and extracellular spaces, while hydrophobic fatty acid tails face one another.
Measurements of the space occupied by individual phospholipids, the depth of the membrane, the size of transient lipid rafts (or, fluidification of the membrane where the lateral spacing between phopholipids is increased) has been accomplished using x-ray diffraction measurements of human red blood cell membrane "ghosts" affixed to silicon layers \cite{himbert2017molecular}.
Interestingly, Asprin alters the structure of the membrane by affixing to phosphate groups and increasing the lateral spacing between phospholipids and fluidifying the membrane \cite{himbert2017molecular}.
In contrast, high pressures can cause the membrane to transition from a fluid-crystaline state to a gel like state (\cite{frey2008cells} and citations therein).
Lipid rafts may organize cytoskeletal assembly by localizing components like PI(4,5)P\_{2} that regulate actin dynamics \cite{caroni2001actin}.
Thus, rafts that mediate a cell's signalling with its external environment and membrane trafficking may also facilitate restructuring of the internal actin architecture \cite{caroni2001actin}, and in turn, the cytoskeleton maintains the spatial separation of rafts \cite{pike2009challenge}.
The size and shape of individual rafts is likely driven by line tension that arises from differences in the depth of the membrane between raft and non-raft regions \cite{pike2009challenge}.

Anionic phospholipids are asymmetrically localized in the membrane in the inner leaflet while the outer leaflet is primarily composed of neutral phospholipids.
The negative charge of the inner leaflet has electrostatic implications \cite{mclaughlin1989electrostatic}, attracting a layer of positively charged molecules to it, and a subsequent layer of negatively charged molecules, which was described by Helmholtz.
The density of these charged molecules can be described with the Guoy-Chapman theory, which takes into account factors such as the diffusivity and charge strength \cite{mclaughlin1989electrostatic}.

One of the early steps of microparticle formation is the redistribution of negatively charged phospholipids into the outer leaflet \cite{PadminiGrant}. 
At rest, negatively charged aminophospholipids [phosphatidylserine (PS) and phospha-tidylethanolamine] are predominately located in the inner leaflet, while phosphatidylcholine and sphingomyelin are enriched in the external one \cite{hugel2005membrane}.
The movement of phosphatidylserine, in particular, from the inner to the outer leaflet upon stimulation is a precursor to microparticle shedding, and also occurs in conjunction with apoptosis \cite{frey2008cells}.
Interestingly, lipid rafts harbor phosphatidylserine and may facilitate its distribution on the outer leaflet \cite{pike2009challenge}.
The asymmetric distribution of phosopholipids in the bilayer is maintained by multiple components: Flippase, Floppase, Scramabase and aminophospholipid translocase \cite{bevers1999lipid}.
Of note, aminophospholipid translocase actively pumps phosphatidylserine and phosphatidylethanolamine to the inner leaflet \cite{bevers1999lipid}.
The movement of negatively charged phospholipids on the inside of the membrane to the exterior when activated by calcium, and changes in calcium concentration also elicit cleavage of the connections of the membrane to the cytoskeleton, decreasing the membrane's rigidity \cite{rubin2012red}. 
I infer that as membrane rigidity is reduced, the change in electrostatics results in a bending force. 
Aim 1 addresses building a multiscale model to investigate this. 

In addition to the asymmetric distribution of lipids between the leaflets, cholesteral localizes asymmetrically,favoring the cytoplasmic leaflet at rest where the lipid chains are more ordered \cite{aghaaminiha2021quantitative}. 

\subsection*{Water and electrical gradients}
Functionally, a membrane is more than the sum of its constituent molecules, exerting longer range effects. 
Near phospholipid heads, water is ordered, but where cations are bound to the negatively charged phospholipid heads water is not ordered. 
The clustered relationships between cations and phospholipid head groups can result in patchiness, where water is ordered in approximately 1.5 $\mu$m domains \cite{tarun2020transient}, and the elctric field loses local symmetry.
In turn, asymmetry in the electrical field across a membrane can exert pressure, elciting membrane curvature \cite{tarun2020transient}.
\textbf{Note:} Almost all of the references in this paper look fascinating.

The charge of the phospholipid head groups can also impact the bending rigidity of the membrane.
In giant unilamellar vesicles (GUVs) membrane rigidity increases with the incorporation of charged phospholipids up to a 20\% density, where the membrane rigidity plateaus \cite{faizi2019bending}. 


\subsection*{Teamwork in extracellular vesicle launch}
Cells need to coordinate the localization of signalling proteins to be packaged in EVs with the molecules necessary to facilitate their release from the membrane. 
For instance, in one study, the release of EVs from the sensory cilia of \textit{C. elegans} containing a channel protein was studied. 
The EVs can be released from both the tip of the cilia, and from the base of the cilia. 
In order to coordinate release from the cilia tip, a variety of players are involved, including a myristoylated coil coiled protein and kinesin motors. 
Fascinatingly, release of these vesicles was stimulated by the presence of potential mates \cite{wang2021sensory}.
\textbf{An idea:} This is a network of interactions -- the number of kinesin motors, for instance, likely effects the probability of EV formation. Does the tuning of this network effect factors like rate of EV release, or size of EVs released? 

%\subsection*{Proteins mediate membrane bending}
%Proteins such as BAR-domain proteins bind to the plasma membrane and induce bending.
%The density of proteins bound to the membrane is balanced by the membrane's tension, resulting in a shape transition that depends on these factors \cite{shi2015membrane}.

\subsection*{Function}
Microparticles can serve as a signal in a multicellular organism, allowing cell membranes to interact across space \cite{morel2011cellular}. 
For instance, since they may be released by cells in one location and circulate through the blood stream (or other fluids) they can serve as effective signals and can raise an immune response \cite{thery2009membrane}. 
For example, exposed phosphotidylserine on the outer leaflet serves as a signal to the immune system to remove the membrane, and it is also procoagulant \cite{hugel2005membrane}.

Microparticles are also released by many cells in the brain and can function as paracrine and autocrine signals. 
At times microparticles carry signals that promote synaptic plasticity and promote connections. 
But they are also involved in deconstruction, in disease, and in signaling inflammation that can go beyond the brain and impact other organs.
These topics are briefly reviewed in \cite{kano2019extracellular}).

Microparticles derived from endothelium, monocytes, B lymphocytes and platelets are positively correlated with Rheumatoid arthritis and modulate inflammation \cite{vinuela2015proportions}.
Microparticles derived from platelets can be found in the synovial fluid \cite{boilard2010platelets}, in addition to plasma and even urine, although it is unknown if microparticles found in the urine arrive there through filtration of plasma, or originate in the urinary tract \cite{vinuela2015proportions}. 
High concentrations of microparticles in the synovial fluid are elicited by the local interactions of the platelet receptor glycoprotein VI with collagen through fenestrated capillaries near the joint. 
In turn, these released microparticles trigger inflammation mediated through interleukin 1 \cite{boilard2010platelets}. 
This looks like a helpful paper on the regulation of interleukin 1 \cite{lindemann2001activated}.

\subsection*{Physics and modeling}
The relative cost of vesicle formation varies with vesicle size, and the weighting of individual mechanisms that resist or contribute to bending, like membrane rigidity and tension, protein crowding, insertions into the membrane, actin polymerization and the addition of coating proteins like clathrin, also vary with vesicle size \cite{stachowiak2013cost}. 
This mechanism is emphasized in a section on microparticle biogensis in this excellent review, along with several others. The papers therin may be useful \cite{tricarico2017biology}. 


This is an excellent resource for the physics of lipid membranes and vesicle topology \cite{seifert1997configurations}.
This review speaks to mathematical modeling of RBC in general, but in section 3 deals specifically with RBC blebbing and vesiculation \cite{li2017computational}.
This paper uses immersed boundary method to model blebbing taking into account fluid flow (Stokes) and membrane - cortex adhesion.
They account for time dynamics, showing how at some initial hole sizes blebs increase in size until a pressure equilibrium is reached, and they summarize their conclusions in phase diagrams demonstrating parameter regimes that result in growing, stable and no-bleb results \cite{fang2017combined}.
This model accounts for membrane tension arising from cortex interaction, membrane stretch and out of plane bending rigidity, however it does not address curvature.
Additionally, potential phase separation and line tension aren't addressed. 

There is this model made available in Python which can be used to model cell blebbing using surface finite element modeling \cite{stinner2020surface}. 
Some limitations are that it doesn't explicitly account for fluid flow, but instead imposes a drag force penalty on membrane motion as a proxy. 
They also don't include variable curvature. 
However this looks like it's very well done and the software is curated at a professional feeling level.
They also include tooling for moving from image data to a finite element model. 

This paper combines theory and experiments with a well done exploration of the poro-elastic nature of the cytoplasm/cytoskeleton \cite{charras2008life}. 
They also go into depth address the retraction of a bleb, which occurs by an inward crumpling of the cytoskeleton towards the cell body, incontrast to a cinching from the inner membrane surface. 
Finally, they also provide a good description of how local cortical contraction results in locally high pressure, facilitating bleb formation, and how in the case of lower pressures, local cortical disassembly or membrane-cortex detachment can permit bleb formation, with a quantification of the tension, bending rigidity, and effective hole sizes necessary for a bleb to form. 

Building from the ideas in \cite{charras2008life}, Lavi \textit{et al.} further considered how tension buffering by tubules in the membrane control blebbing probability \cite{lavi2019cellular}. 
They elucidate that as the density of N-BAR proteins increases, membrane is stabilized in tubules. 
Bleb formation depends on "taking up the slack" in the membrane and flattening out these tubules (which entails dispersing aggregations of N-BAR), so overexpression of N BAR results in decreased bleb formation. 
However, increasing the acto-myosin contractility (which is posited to increase hydrostatic pressure) can restore bleb frequency to wildtype frequency, and even beyond.

Have yet to read this paper, but it incorporates fluid flow and Helfrich, and appears to be imperative to consider \cite{werner2020pde}. 
Kindly, fate smiled on me, and it was cited by \cite{stinner2020surface}, so it would be interesting to see what their commentary was since they do not account for fluid flow. 
Further, this model \cite{dirks2021mathematical} also cites \cite{werner2020pde}.
While the final paper is paywalled, they appear to have largely made similar assumptions according to bioarchive drafts. 

Another line of modeling is particle based simulations. 
Coupling a lipid bilayer (without intrinsic curvature or lipid diversity) with an elastic cytoskeletal network reminescent of the RBC's spectrin network Spangler \textit{et al.} found that area mismatch between the bilayer and cytoskeleton facilitates bleb formation, and that as with decreasing gap size (corral size) in the cytoskeleton, the area mismatch needed to spur bleb formation grows \cite{spangler2011computer}.
They also show how a vesicle with many blebs eventually consolidates to fewer blebs as simulation time goes on. 
In their introduction they speak to the small vesicles that bud from RBCs and hypothesize that these may be facilitated by the corral size of the spectrin network. 
This model does not account for fluid flow. 

\subsection*{Vesicles and protocells}
Investigation into the early origins of life has shown a spotlight on the biophysics of vesicles since compartmentalization is supposed to be a fundamental step in the origins of cellular life by confining metabolic and information processing reactions to a small space and increasing their probability  \cite{deamer2002first,sole2009evolution}. 
Dissipative Particle Dynamics is a coarse grained modeling method that describes the interaction of water, phospholipid heads and phospholipid tails as "beads".
Beads can interact in space over a prescribed difference, random motion can be added to account for thermal fluctuation, dissipation describing viscosity can be incorporated and beads are allowed to interact with neighbors with a strength prescribed based upon their pair wise identity, and covalent bonds are modeled as harmonic spring force \cite{sole2009evolution}.
By using this model, Sole \textit{et al.} demonstrated that the size of fission products depends on the hydrophobicity of the surfactant.
A question that follows from this is does microparticle size depend on 1) phospholipid shape and 2) the hydrophobicity of the phospholipid.
This may connect to the flipping of negatively charged aminophospholipids to the external leaflet. 

\subsection*{Some basic physics}
The Young-Laplace equation relates the pressure difference ($\Delta P$) across an interface, the coefficient of surface tension ($\gamma$), and the radii of curvature ($R_{1}$ and $R_{2}$) by: 
\begin{equation}
\Delta P = \gamma \left( \frac{1}{R_{1}} +  \frac{1}{R_{2}} \right)
\end{equation}
This relationship applies for a single interface, such as a gas bubble within a fluid. 
However, for a phospholipid bilayer there are multiple interfaces to consider: extra-vesicular fluid, the thin lipid core and the intra-vesicular fluid. 
For two the case where the inner and outer radii are close to one another, there is a simple approximation (see the Wikepedia article on Laplace pressure). 
However, given that the total depth of the lipid bilayer may not be much smaller than the a small microparticle's radius, I am wary of about the validity of this type of approximation. 

The shape of the phospholipids influences the shape of resulting structures. 
When the hydrophilic end is relatively small micelles are formed. 
As the volume of the hydrophilic end grows relative to the hydrophobic end, lipids tend to form flat bilayers, then connected cylindrical networks, and finally, vesicles surrounded by a phospholipid bilayer \cite{sole2009evolution}. 

\subsection*{Membrane shape can be driven by proteins}
A sufficient mechanism to induce membrane curvature is tight packing of protein on a membrane domain. 
Stachowiak \textit{et al.} demonstrate that the binding of GFP to a phase separated lipid regions on a Giant Unilamellar Vesicle is sufficient to induce membrane puckering, budding and tubule formation, indicating that protein crowding alone can cause membrane deformations \cite{stachowiak2010steric}.

Proteins with transmembrane components can also curve the lipid bilayer if their distribution is asymmetric.
For instance, in the Endoplasmic Reticulum the REEP family of proteins dimerise, their components splaying out on the exterior portion of the bent bilayer \cite{wang2021mechanism}.
Transmembrane proteins can also oligorimize forming a scaffold that bends the membrane as in the case of BAR proteins \cite{boucrot2012membrane}.
Proteins such as BAR-domain proteins bind to the plasma membrane and induce bending.
The density of proteins bound to the membrane is balanced by the membrane's tension, resulting in a shape transition that depends on these factors \cite{shi2015membrane}.

\subsection*{Membrane shape can be driven by the glycocalyx}
The glycocalyx has also been demonstrated to play a role in tubule formation and vesicle formation. 
These polymers which attach to the membrane can pack densely, with a phase transition from a coiled disposition at relatively low densities to a highly ordered brush state, and their packing can induce steric repulsion and, consequently, membrane curvature. 
This transition point marks a pivotal energetic turning point between the formation of blebs and tubules \cite{shurer2019physical}.
Further, the diameter of long tubules formed in cells with a dense glycocalyx is determined by actin filaments.
If actin filaments are dissassembled, the preferred membrane curvature of the polymer coat results in an array of preferred topologies from cylindrical to consistently, or even variably sized, pearls. 
The tightly constricted membrane necks along a pearl chain allow for favorable vesiculation, correspondingly, experimental results demonstrate the formation of microparticles in this manner \cite{shurer2019physical}.
This mechanism may have widespread prevalence, as their is a correlation between cell types known for their formation of tubules and microparticles and those known for their glycocalyx \cite{shurer2019physical}.

\subsection*{Attachment of proteins to the membrane}
Transmembrane proteins can be attached to the membrane during their production, or they can insert after translation.
As an example, myristoylated proteins (which are proteins where a fatty acid myristoyl group is added, either at translation or post-translation) have a small energetic bias for their tails to integrate into the membrane, but it is small enough that factors like electrostatic repulsion between the phospholipid heads of the membrane and the protein could prevent association \cite{peitzsch1993binding}. 

\subsection*{Membrane fission}
\subsubsection*{Exocytosis}
What are the necessary components of membrane fission?
The release of virus particles from the host membrane is one system where this question has been evaluated. 
The following observations come from a wonderful review: \cite{weissenhorn2013get}.
Some viruses use host cell machinery, like the ESCRT complex to leave the host cell.
Although the ESCRT machinery's involvement in endosomal transport and in the shedding of some viruses, how ESCRT accomplishes the separation of the neck is not yet clear. 
While proteins like ESCRT play critical roles, \textit{in vitro} studies have demonstrated that line tension in the membrane and lipid phase transitions are enough to yield fission.
Interestingly, these biophysical mechanisms can also work in tandem. 
Other mechanisms, like the formation of protein coats that wrap the whole viral membrane, or the actions of proteins like M2 in the influenza virus which interact with membrane cholesteral to induce bending are also prominent players in scission.

\subsubsection*{Endocytosis}
In clathrin mediated endocytosis, both dynamin (a GTPase) and actin have been suggested as mediators of fission. 
Both of these proteins localize at clathrin coated structures (CCSs) during the late stages of endocytosis as demonstrated by fluoresence microscopy, although neither has been observed with electron microscopy, possibly because their structures form and dissipate so quickly. 
In fact, dynamin may orchestrate the formation of actin filaments around vesicles, while actin (and potentially myosin) provide force propelling vesicles into the body of the cell \cite{merrifield2002imaging}.
While dynamin has been shown to be an active participant in many types of endocytosis, it is not necessary for the fission of intracellular vesicles. 
Hence it may be concluded that it is a key regulator of endocytosis, but its exact mechanism remains unclear \cite{conner2003regulated}. 
Additionally, it endocytosis can occur independently of dynamin (a paper I've not read but is likely good: Sathe, Mugdha, et al. "Small GTPases and BAR domain proteins regulate branched actin polymerisation for clathrin and dynamin-independent endocytosis." Nature communications 9.1 (2018): 1-16.)


\subsection*{Intracellular vesicle transport}
How do vesicles reach their target sites? 
In oocytes, cortical granules formed by the golgi at the cell's center must be anchored in the cell's cortex during oocyte maturation. 
Experimental results show that their transport is facilitated by actin, but not by microtubules \cite{cheeseman2016two, wessel2001biology}. 
Both by association with Rab11a vesicles, and directly with myosin molecular motors, cortical granules are reliably transported from the cell's center and docked near the membrane \cite{cheeseman2016two}.
Incidentally, Rab GTPase proteins play critical roles in vesicle trafficking across myriad (dare I say all?) cell types that I'm not well versed in.  
The dense actin cortex, along with myosin, is locally disassembled, allowing cortical granule exocytosis \cite{vogt2019anchoring}.

Directed transport along microtubule tracks may be a mechanism that enables transport to occur more effectively than diffusion, or the random movement along an undirected microtubule network. 
These questions have been investigated using an agent based model \cite{klann2012spatial}.

\subsection*{Membrane tension}
Membrane tension regulates cell state transitions.
Cells which are spreading use plasma membrane stored in ruffles, invaginations, \textit{etc.} to increase their surface area.
But as the pool of available membrane is used up the tension of the membrane is increased, which drives more membrane from the cell's interior to be exocytosed and joined with the exterior plasma membrane. 
Increased membrane tension also spurs actomyosin contractility, facilitating cell adhesion \cite{gauthier2011temporary}. 

The formation of blebs and pseudopods in migrating cells can act as feedforward loop since regions of negative curvature (concave) along the membrane facilitate bleb formation as the normal component of membrane tension is directed outward, rather than inward \cite{tyson2014blebs}.
Further, Collier \textit{et al.} used a 2D computational model of the membrane use contours from migrating cell images to predict where blebs would form and compare this to the sites of actual blebbing, finding that the curvature of the membrane is a good predictor of bleb sites in rounded cells. 
In cells with a more elongated geometry the model was not as predictive, however the addition of a polarized cortex-membrane adhesion strength (modeling Talin distributions observed experimentally) improved the model's predictivity for the elongated case and didn't change its predictivity for the rounded case \cite{collier2017image}.
Indeed, bleb formation depends on the cell reaching a critical tension point \cite{tinevez2009role}. 
Further, Tinevez \textit{et al.} used an experimental set up to demonstrate that the pressure drop from a bleb on one side of a cell rapidly propagates so that a bleb induced by laser ablation of the cortex on the opposite side of the cell is much smaller. 
They also created a model where they posit a balance between the cytoskeletal elasticity and membrane tension, estimating the critical tension at which blebs form \cite{tinevez2009role}. 

\subsection*{Role of the cortex in microparticle formation}
The plasma membrane is tethered to the cortex, which lends effective tension and rigidity to the membrane.
Phosphatidyli-nositol  4,5-bisphosphate (PIP$_{2}$), a phospholipid comprising \~ 1\% of the membrane, is a key regulator of cortex-membrane interactions, among other functions \cite{jaxnmey2018regulation}.
An increase in PIP$_{2}$ concentration in the membrane prevents microparticle formation in platelets, and calpain has been found to reduce PIP$_{2}$ concentration, facilitating microparticle formation  \cite{o2005phosphatidylinositol}.  
Importantly, calpain augments microparticle formation both deconstructing the cytoskeleton, and by effecting the concentration of PIP$_{2}$ independent of the break down of the cortex. 
These results demonstrates that membrane phospholipids are regulators of microparticle formation, and that microparticles can form independent of cytoskeletal degredation \cite{o2005phosphatidylinositol}.

Since PIP$_{2}$ is an important regulator of membrane cortex attachment, the question of where it localizes emerges.
The diffusion of PIP$_{2}$ is slower on the inner than the outer leaflet and blebs, and PIP$_{2}$ is in fact depleted in microparticles \cite{}.
Approximately two thirds is sequestered near clusters of basic proteins, while one third is free to diffuse \cite{golebiewska2008diffusion}.
The amount of freely PIP$_{2}$ sequesterd can be regulated by basic protein clusters, which are co-located with cell structures like ruffles (verify this statement with Sheetz's work) \cite{}.

Membrane organization is also inextricably linked to the organization of the cortex, with aster formations in the cortex colocalizing with organized lipid rafts in the membrane, even while structures like actin stars do not \cite{fritzsche2017self}.
While it is well known that the cortex is vital to membrane order (see citations within \cite{fritzsche2017self}), I wonder if it is understood how diffusion of membrane rafts and protein aggregation couple with cortical remodeling. Were the cortex to be fixed, what modifications in membrane function would we observe?

Ezrin, radixin and moesin are proteins that anchor the membrane to the cortex when activated by phosphorylation.
They are often called as the ERM family since each accomplishes membrane-cortex attachement in different tissues: ezrin in the epithelium, radixin in hepatocytes and moesin in the endothelium \cite{fehon2010organizing}.
The genes encoding these proteins are located on different chromosomes, and while they have similar functional roles, it has not been established whether they are identical or not. 
During mitosis the cell rounds, which may result from the concomitant alignment of actin filaments in parallel with the membrane and the increase of membrane stiffness. 

Interestingly, if Moesin is inhibited in \textit{D. Melanogaster} mitotic cells are unable to round up, display mislocalization of RhoA and they bleb extensively (Verify this in this paper: https://rupress.org/jcb/article/180/4/739/53708). 
While blebs in this case result from Moesin's inhibition, bleb retraction is also mediated by activated Moesin. 

A vital question is how does the plasma membrane at the cite of a microparticle release from the cortex. 
Often, the acto-myosin cortex is disassembled by calcium influx that triggers calpain proteolysis, and so the cytoskeleton is remodeled in tandem with microparticle release \cite{pasquet1996calcium}.
While the temporal dynamics of cortex disassembly correlate with microvesicle release, Wiedmer \textit{et al.} demonstrate that in platelets microparticle release can occur independent of cortex disassembly when they are stimulated by c5b-9 \cite{wiedmer1990role}, although generally calpain inhibition prevents platelets from releasing microparticles as reviewed by \cite{randriamboavonjy2012all}.
Further, the inhibition of calpain (via calpeptin) both reduces MP production in platelets and stabilizes long filopodial protrusions constructed by activated platelets \cite{basse1994correlation}.
Basse \textit{et al} further demonstrated that platelets exposed to large quantities of calpeptin do still, in fact, form some MPs.
However, these MPs contain high molecular weight proteins. 
They speculated that the origin of these MPs may be fragments of fiolopods (the size and number of which are positively correlated with calpeptin dose) that contain undegraded cortex components, and that in fact this may be the mechanism by which platelts stimulated by c5b-9 may still release MPs despite calpain inhibition \cite{basse1994correlation}. 
These observations on the interaction of the cortex and membrane raise interesting modeling possibilities -- does cortex disassembly influence the size of a microparticle? Does cortex disassembly influence the probability of producing a microparticle? 
While Wiedmer \textit{et al.} produce incisive results, the use of bulk analytics that they were constrained to in the 80s rather than time resolved single cell studies that can now be accomplished reduces the conclusions that can be made about microparticle size and the likelihood of microparticle formation. 



\subsection*{Sage's ongoing questions}
The cortex beneath the membrane is possibly quite dense with minimal space between actin filaments. 
What are the largest vesicles synthesized by the ER system which must be transported through this meshwork?
What are the drag forces on those vesicles? 
To what extent is clearing around a vesicle possible? 
Alternatively, might there be nucleation of actin around the vesicle -- could this apply further forces to the vesicle, pushing it against the membrane as the interior vesicle grows close to the membrane (directed motion on microtubules)? 
Alternatively, could there be greater contraction of the cytoskeleton on the cell side of the microparticle then the membrane side (where the space is physically occluded by the vesicle)?
If a vesicle is on a microtubule track pulled by dynenin/kinesin, what force could that alone produce? 
\newline

\subsection{Applications for muscle and exercise}
Recent work indicates that motor neuron boutons are formed by a pressure driven blebbing mechanism, rather than actin polymerization driven protrusions \cite{fernandes2021motor}.
Further, they demonstrate that increased muscle contraction spurs the development of boutons, positing that the confinement of motor neurons embedded in a contracting muscle leads to higher pressure/tension. 
This paper is as yet a Bioarxive submission, so I'm interested to see how it shapes up after publication. 

This paper lays out a review of the composition of MPs and extracellular vesicles released by myoblasts and myotubes with some discussion of their functional implications in exercise and metabolic disease \cite{rome2019skeletal} (Incidentally, Sophie Rome has several publications about extracellular vesicles from adipocytes and plant cells, also). 

Muscle cells release extracellular vesicles in response to excercise which vary in composition depending on the type of excercise. 
The functional significance of excercise spurred microparticle release is an emerging research area \cite{vechetti2021role}.

This paper on exosomes participating in adaptation to endurance excercise looks interesting \cite{safdar2018exosomes}.

\PR{Arijit, can we do any kind of stability analysis? or at least obtain dimensionless parameters to give insight into the model?
What is it that is new here?}
\subsection*{Effect of point force and relaxation dynamics of the membrane}
We first investigate the relaxation dynamics of the membrane in response to a locally applied point force. 
\PR{I only see two lines in this figure so I can't figure out where the spontaneous curvature is.
This might end up being a supplementary figure.}

\subsection{Effect of feedback}
\PR{We should discuss the details of how this was done.}

\subsection{Effect of membrane properties on microparticle formation}

Numerous studies have shown that membrane properties including tension and bending modulus can affect the curvature generation capabilities of the membrane \needref.
We next investigated how the formation of MPs, especially the linker detachment could be affected by these properties. 
To do this, we simulated the induction of spontaneous curvature using PS kinetics as in Eq \PR{crossref} and linker kinetics using Eq \PR{crossref}. 
We first fixed the value of the bending modulus to $\kappa=90 k_BT$ \PR{need to discuss value, why?} and varied tension over three values \PR{Arijit, insert values.}
\PR{Arijit, some questions that come up especially with the linker density. For high tension, why does it increase? Is it because you are starting at a low value of linker density and because of the rate constants, it is going to a steady state? The linker values going up suggests that the linkers are rebinding. What values did you use for kon and koff? Did you ever vary those? In all your deformations, where would expect the linker density to be zero, we are seeing high linker density. that is probably a weird rebinding thing going on. I don't understand it. We should discuss. }

\begin{itemize}
    \item Figure 2: estimation of spontaneous curvature of the membrane due to PS flipping -- see the Nat comms Hirama 2017 et al. Adapt their model to yours. use bending modulus from the other paper I sent you.
    \item Figure 3: simple bending model with no pressure -- under what combination of reasonable parameters do you get buds? Tension, bending modulus, spontaneous curvature, and area of the curvature are the variables here. Pick results from your training data set to inform this figure. you will also want to consider plotting the energy.
    
    I think a result that could be discussed in this section is the "patchiness" of parameter space
    
    \item Figure 4: what happens when you add pressure to the results in Figure 3?
    
    From the ML paper I believe that pressure will be most important for restoring omega shapes for large MPs.
    
    \item Figure 5: and what happens when you add adhesion energy?  
    
    Hopefully adhesion will help tack  the membrane down and encourage a neck to form. 
\end{itemize}

The goal is to extract how lipid composition and charge distribution combined with cortical actin and fluid pressure alter the bending landscape.
